ProtoMed-LLM: An Automatic Evaluation Framework for Large Language Models in Medical Protocol Formulation

Automated generation of scientific protocols executable by robots can significantly accelerate scientific research processes. Large Language Models (LLMs) excel at Scientific Protocol Formulation Tasks (SPFT), but the evaluation of their capabilities rely on human evaluation. Here, we propose a flexible, automatic framework to evaluate LLMs' capability on SPFT: ProtoMed-LLM. This framework prompts the target model and GPT-4 to extract pseudocode from biology protocols using only predefined lab actions and evaluates the output of the target model using LLAM-EVAL, the pseudocode generated by GPT-4 serving as a baseline and Llama-3 acting as the evaluator. Our adaptable prompt-based evaluation method, LLAM-EVAL, offers significant flexibility in terms of evaluation model, material, criteria, and is free of cost. We evaluate GPT variations, Llama, Mixtral, Gemma, Cohere, and Gemini. Overall, we find that GPT and Cohere are powerful scientific protocol formulators. We also introduce BIOPROT 2.0, a dataset with biology protocols and corresponding pseudocodes, which can aid LLMs in formulation and evaluation of SPFT. Our work is extensible to assess LLMs on SPFT across various domains and other fields that require protocol generation for specific goals.

==> 5.tex <==
\begin{table*}[htbp!]
%\footnotesize % Reduce the font size to 'footnotesize'
\centering
\setlength{\tabcolsep}{4pt} % Reduce space between columns
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l|cccc|cc}
\toprule
 & \multicolumn{4}{c|}{Original Criteria} & \multicolumn{2}{c}{New Criteria} \\
Models & Coherence & Consistency & Fluency & Relevance & Precision & Coverage \\ 
\midrule
GPT-3.5 & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
GPT-4   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
GPT-NeoX   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
\midrule
Gemini-1.0 Pro   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
Gemini-1.5 Pro   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
Gemini-1.5 Pro   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
% \midrule
% PaLM   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
% \midrule
% BERT   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
% \midrule
% T5   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
\bottomrule
\end{tabular*}
\caption{\textbf{Protocol - Pseudocode Evaluation} We report mean and standard deviation of scores over five runs. The best and second best performance for each criterion is bolded and underlined, respectively. Higher values for all metrics represent better performance.}
\label{tab:results-2}
\end{table*}


==> 7.tex <==
% \begin{table*}[htbp!]
% %\footnotesize % Reduce the font size to 'footnotesize'
% \centering
% \setlength{\tabcolsep}{4pt} % Reduce space between columns
% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l|cccc|cc}
% \toprule
%  & \multicolumn{4}{c|}{Original Criteria} & \multicolumn{2}{c}{New Criteria} \\
% Models & Coherence & Consistency & Fluency & Relevance & Precision & Coverage \\ 
% \midrule
% GPT-3.5 & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
% GPT-4   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
% GPT-NeoX   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
% \midrule
% Gemini-1.0 Pro   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
% Gemini-1.5 Pro   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
% Gemini-1.5 Pro   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
% % \midrule
% % PaLM   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
% % \midrule
% % BERT   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
% % \midrule
% % T5   & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ & $.00 \pm .00$ \\
% \bottomrule
% \end{tabular*}
% \caption{\textbf{Pseudocode - Pseudocode Evaluation} We report mean and standard deviation of scores over five runs. The best and second best performance for each criterion is bolded and underlined, respectively. Higher values for all metrics represent better performance.}
% \label{tab:results-code-code}
% \end{table*}

